Coding and System Design for Quantize-Map-and-Forward Relaying

In this paper we develop a low-complexity coding scheme and system design framework for the half duplex relay channel based on the Quantize-Map-and-Forward (QMF) relay- ing scheme. The proposed framework allows linear complexity operations at all network terminals. We propose the use of binary LDPC codes for encoding at the source and LDGM codes for mapping at the relay. We express joint decoding at the destination as a belief propagation algorithm over a factor graph. This graph has the LDPC and LDGM codes as subgraphs connected via probabilistic constraints that model the QMF relay operations. We show that this coding framework extends naturally to the high SNR regime using bit interleaved coded modulation (BICM). We develop density evolution analysis tools for this factor graph and demonstrate the design of practical codes for the half-duplex relay channel that perform within 1dB of information theoretic QMF threshold.

==> Sysarc.tex <==
%
% SVN properties (Automatically populated)
% Last changed by $Author: vnagpal $
% Last changed $Date: 2010-10-04 11:31:22 -0700 (Mon, 04 Oct 2010) $
% Last changed $Revision: 373 $
% Summary $Id: Sysarc.tex 373 2010-10-04 18:31:22Z vnagpal $
%

%\subsection{System Architecture}
%The system architecture is depicted in Figure . It is a three terminal system with one source terminal, one relay terminal, and one destination terminal. 

%In this paper we focus on the half duplex Gaussian relay channel, depicted in Figure \ref{fig_HDR}. It consists of three half-duplex terminals: source (S), relay (R), and destination (D), and the signals received at the R and D terminals are
%\begin{align}
%y_{R} &= \mb{H}_{R}x + z_{R}\\
%y &= \mb{H}_1x + \mb{H}_2x_{R} + z
%\end{align}
%respectively, where the signals are all complex vectors with dimensions matching the numbers of antennas at the corresponding terminals. The noises are independent 

%\begin{figure}[htbp]
%{\center
%%\subfigure[Original Gaussian Downlink Scenario]{\includegraphics[width=3in]{Gaussian_DL_primary.pdf}}
%\includegraphics[width=3in]{HDRelayChannel.pdf}
%\caption{Half-Duplex Gaussian Relay Channel}
%\label{fig_HDR}
%}
%\end{figure}
\subsection{DBLAST Architecture}
\label{sec_dblast}
%\begin{figure*}[htbp]
%{\centering
%%\subfigure[Original Gaussian Downlink Scenario]{\includegraphics[width=3in]{Gaussian_DL_primary.pdf}}
%\includegraphics[width=5in]{SysArch.pdf}
%\caption{System architecture for block index $b$.}
%\label{fig_SysArch}
%}
%\end{figure*}

%In this section we outline a layered space time architecture for the relay channel based on 
DBLAST (diagonal Bell-Labs space-time) was originally introduced for MIMO channels to allow coding across antennas for slow fading scenarios. The relay channel can be thought of as a distributed MIMO channel with coding across the transmit antennas (source and relay). This is a natural fit for the relay channel and we show that it provides several system design advantages. The equivalent channel model is shown in Fig.~\ref{fig_EquivCh}.  The architecture relies on introducing a delay of one block at the relay. At the $b$-th block the destination receives the superposition of the following:
\begin{itemize}
\item signal from the source containing the codeword sent at block $b$, namely, $\mb{x}_{S}(m_b)$
\item signal from the relay containing the side information about the source's codeword at block $b-1$, namely, $\mb{x}_{R}(q_{b-1})$
\end{itemize} 
Across blocks the messages sent from the source are independent and the destination can perform successive interference cancellation (SIC).  At the $b$-th block, it jointly decodes block $b-1$ (message $m_{b-1}$ and side information $\mb{x}_{R}(q_{b-1})$) by treating $\mb{x}_{S}(m_b)$ as Gaussian noise. Then it subtracts relay's codeword $\mb{x}_{R}(q_{b-1})$ from its received signal $\mb{y}[b]$ and keeps the residual $\mb{\wtild{y}}[b]$ for decoding the next block. This architecture allows us to use a simplified equivalent channel model.
{\flushleft \it Simplified Equivalent Channel Model}:\par 
%\subsubsection{Simplified Channel Model:} 
%\label{subsec_ECM}
For decoding the block $b-1$ message $m_{b-1}$, the decoder takes two inputs $\mb{y}[b]$ and $\mb{\wtild{y}}[b-1]$. Note that the noises are independent over time and the messages sent at all blocks are independent. We can think of $\mb{y}[b]$ and $\mb{\wtild{y}}[b-1]$ as two orthogonal links with independent additive Gaussian noises. Therefore, for the purpose of code design we can alternatively investigate a simpler model depicted in Figure \ref{fig_EquivCh}. In this model,
\begin{align*}
y_{ij} &= h_{ij}x_{i} + z_{ij},\ (i,j)=(S,R), (R,D), (S,D),
%y_{SR} &= h_{SR}x_{S} + z_{SR}\\
%y_{SD} &= h_{SD}x_{S} + z_{SD}\\ 
%y_{RD} &= h_{RD}x_{R} + z_{RD}
\end{align*}
where $h_{SR} = h_{R}$, $h_{SD} = h_1$, $h_{RD}=h_2$, and $z_{SR}$, $z_{SD}$, and $z_{RD}$ are independent Gaussian noises with variances
\begin{align*}
\Var[z_{SR}] = \Var[z_{SD}] = 1,\ \Var[z_{RD}] = 1+|h_1|^2.
\end{align*}
The equivalent noise $z_{RD}$ has higher variance since the signal from the source in block $b$ is treated as Gaussian noise. We denote the signal-to-noise ratios in the three links by $\SNR_{SR}$, $\SNR_{SD}$, and $\SNR_{RD}$ respectively. %In general, $\SNR_{SD}$ and $\SNR_{RD}$ are related since in the system we 

\begin{figure}[htbp]
{\center
%\subfigure[Original Gaussian Downlink Scenario]{\includegraphics[width=3in]{Gaussian_DL_primary.pdf}}
\includegraphics[width=2.5in]{EquivCh.pdf}
\caption{Equivalent channel model}
\label{fig_EquivCh}
}
\end{figure}

\begin{remark}
Consider the original channel and the equivalent channel under DBLAST \emph{without} binary input constraint i.e. average power constraint is put at the transmitters. It is not difficult to show that the capacities of these two channels are within a constant gap. Note that the cut-set upper bounds for both channels are within $1$ bit (for any listening time $f\in[0,1]$). Compared with the original channel in Fig.~\ref{fig_HDR}, the cut at the source remains unchanged, while the cut at the destination has a $\lb (1-f)\times 1\rb$-bit power-gain loss since SIC achieves the sum capacity of multiple-access channels, and this cut in the original channel allows full cooperation of $S$ and $R$. Since QMF achieves the cut-set bound to within a constant gap for arbitrary half-duplex Gaussian relay networks, the capacities are within a constant gap. Therefore for our original purpose of implementing QMF, such DBLAST architecture does not incur much loss.
\end{remark}
%It is worthwhile noting that the cutset bounds of the two channels in Figure \ref{fig_HDR} and Figure \ref{fig_EquivCh} are the same, and hence the capacities are within a constant gap. Let $C$ and $C_{\rm{DBLAST}}$ denote the capacities of the original channel and the equivalent channel under DBLAST. 
%\begin{theorem}
%$\big\lvert C - C_{\rm{DBLAST}} \big\lvert \le 1$ bit. 
%\end{theorem}
%\begin{proof}
%A cut-set upper bound for the original relay channel is 
%\end{proof}


%\subsection{BICM Decomposition:} Consider the equivalent channel model without the binary-input constraint.












==> fig/FactorGraph3.graffle/.svn/entries <==
10

dir
632
svn+ssh://intelr900-1.eecs.berkeley.edu/tools/designs/Dcdg/users/CollMIMO/svn/coopmimo/papers/allerton2010/src/fig/FactorGraph3.graffle
svn+ssh://intelr900-1.eecs.berkeley.edu/tools/designs/Dcdg/users/CollMIMO/svn



2010-06-09T05:15:32.950011Z
305
vnagpal


svn:special svn:externals svn:needs-lock











28a903b5-2779-0410-bdb3-e814c9e2e338






0

Icon\x0d
file

svn+ssh://intelr900-1.eecs.berkeley.edu/tools/designs/Dcdg/users/CollMIMO/svn/coopmimo/papers/allerton2010/src/fig/FactorGraph3.graffle/Icon%0D


2010-06-08T09:24:04.000000Z
d41d8cd98f00b204e9800998ecf8427e
2010-06-08T09:30:14.671566Z
298
ihsiang





















0

data.plist
file




2010-06-09T07:38:37.000000Z
39d27cb57404d6931697ba4f0a0274a8
2010-06-09T05:15:32.950011Z
305
vnagpal





















423265

image10.pdf
file




2010-06-08T09:24:04.000000Z
7dcb4e580fbe3d35bf08d8125680bf39
2010-06-08T09:30:14.671566Z
298
ihsiang
has-props




















11378

image11.pdf
file




2010-06-08T09:24:04.000000Z
16577406caafd0bf48e83ea1a8e4bad1
2010-06-08T09:30:14.671566Z
298
ihsiang
has-props




















16456

image12.pdf
file




2010-06-08T09:24:04.000000Z
a28dadbefef0d15bddf47c1e3199063c
2010-06-08T09:30:14.671566Z
298
ihsiang
has-props




















18960

image14.pdf
file




2010-06-08T09:24:04.000000Z
83b7e6847212ad8362e39208feac5462
2010-06-08T09:30:14.671566Z
298
ihsiang
has-props




















44061

image3.pdf
file




2010-06-08T09:24:04.000000Z
ec9fd3e4f061c863f42bbb0b9dc69f1d
2010-06-08T09:30:14.671566Z
298
ihsiang
has-props




















19438

image4.pdf
file




2010-06-08T09:24:04.000000Z
530755b156f98bee59adbd1466ee2cf2
2010-06-08T09:30:14.671566Z
298
ihsiang
has-props




















16779

image5.pdf
file




2010-06-08T09:24:04.000000Z
3590f26c62670a6b32e95d365cd11be2
2010-06-08T09:30:14.671566Z
298
ihsiang
has-props




















11771

image6.pdf
file




2010-06-08T09:24:04.000000Z
2cf9dbb8f882661fada12b7402603cfd
2010-06-08T09:30:14.671566Z
298
ihsiang
has-props




















11966

image7.pdf
file




2010-06-08T09:24:04.000000Z
6d9cfa1bb6ae3e4ab2f591ee3987e99a
2010-06-08T09:30:14.671566Z
298
ihsiang
has-props




















11500

image8.pdf
file




2010-06-08T09:24:04.000000Z
f36a9de815b065a24282acdef07bad05
2010-06-08T09:30:14.671566Z
298
ihsiang
has-props




















11460

image9.pdf
file




2010-06-08T09:24:04.000000Z
5bf257e1b06ea1d338b55f791ccd3d1d
2010-06-08T09:30:14.671566Z
298
ihsiang
has-props




















11337



==> fig/HDRelayChannel.graffle/.svn/entries <==
10

dir
632
svn+ssh://intelr900-1.eecs.berkeley.edu/tools/designs/Dcdg/users/CollMIMO/svn/coopmimo/papers/allerton2010/src/fig/HDRelayChannel.graffle
svn+ssh://intelr900-1.eecs.berkeley.edu/tools/designs/Dcdg/users/CollMIMO/svn



2010-06-06T06:03:10.640993Z
275
vnagpal


svn:special svn:externals svn:needs-lock











28a903b5-2779-0410-bdb3-e814c9e2e338






0

Icon\x0d
file

svn+ssh://intelr900-1.eecs.berkeley.edu/tools/designs/Dcdg/users/CollMIMO/svn/coopmimo/papers/allerton2010/src/fig/HDRelayChannel.graffle/Icon%0D


2010-06-01T09:54:23.000000Z
d41d8cd98f00b204e9800998ecf8427e
2010-06-01T10:43:57.332216Z
270
ihsiang





















0

data.plist
file




2010-06-06T06:23:59.000000Z
92bb3080312d5dfc35c8612cee1aa03d
2010-06-06T06:03:10.640993Z
275
vnagpal
has-props




















492269

image10.pdf
file




2010-06-01T09:54:22.000000Z
ac2722457d2f4d6e689e879172f8847f
2010-06-01T10:43:57.332216Z
270
ihsiang
has-props




















28194

image11.pdf
file




2010-06-01T09:54:22.000000Z
c6f7f0f8cf7f71774979ce02d4b3e6f7
2010-06-01T10:43:57.332216Z
270
ihsiang
has-props




















28203

image12.pdf
file




2010-06-01T09:54:22.000000Z
07998a3114e17f9ff2325d7b39aa0fd4
2010-06-01T10:43:57.332216Z
270
ihsiang
has-props




















20408

image13.pdf
file




2010-06-01T09:54:22.000000Z
28a497f0b34c6abaf5fb94ec88dd8427
2010-06-01T10:43:57.332216Z
270
ihsiang
has-props




















20411

image14.pdf
file




2010-06-01T09:54:22.000000Z
b28815a0405d12f8e7c0a019077eb770
2010-06-01T10:43:57.332216Z
270
ihsiang
has-props




















28178

image17.pdf
file




2010-06-01T09:54:22.000000Z
004302c996cced7423133121f94067c1
2010-06-01T10:43:57.332216Z
270
ihsiang
has-props




















43634

image18.pdf
file




2010-06-01T09:54:22.000000Z
d10856758179845baad3260b7face9f9
2010-06-01T10:43:57.332216Z
270
ihsiang
has-props




















43397

image19.pdf
file




2010-06-01T09:54:22.000000Z
331a2c9c2977ac17e0199575d61e3220
2010-06-01T10:43:57.332216Z
270
ihsiang
has-props




















43450

image21.pdf
file




2010-06-01T09:54:22.000000Z
e5059c755d7d46ecbf700d96ae27d5b8
2010-06-01T10:43:57.332216Z
270
ihsiang
has-props




















28114

image22.pdf
file




2010-06-01T09:54:22.000000Z
4e8e4a82df8ae205732a14021a56fd48
2010-06-01T10:43:57.332216Z
270
ihsiang
has-props




















28162

image23.pdf
file




2010-06-01T09:54:22.000000Z
8c792ab7ddaf26eac94e6efcd0370e72
2010-06-01T10:43:57.332216Z
270
ihsiang
has-props




















28054

image24.pdf
file




2010-06-01T09:54:22.000000Z
1b1ea0528390e335850607a76e1a35b3
2010-06-01T10:43:57.332216Z
270
ihsiang
has-props




















43609

image25.pdf
file




2010-06-01T09:54:22.000000Z
4a189358bfbb092c2e5ccabd68dbeecb
2010-06-01T10:43:57.332216Z
270
ihsiang
has-props




















59544

image26.pdf
file




2010-06-01T09:54:22.000000Z
66a41c4ed8b2c6dd8bc11e692f788f29
2010-06-01T10:43:57.332216Z
270
ihsiang
has-props




















35610

image27.pdf
file




2010-06-01T09:54:22.000000Z
c82c11091d716379b5703330bf80804b
2010-06-01T10:43:57.332216Z
270
ihsiang
has-props




















35666

image28.pdf
file




2010-06-01T09:54:22.000000Z
3c3842192a835760c72d3ea418f9bd61
2010-06-01T10:43:57.332216Z
270
ihsiang
has-props




















51746

image29.pdf
file




2010-06-01T09:54:22.000000Z
9ac78a28ccffb6877c2244ddd7e61711
2010-06-01T10:43:57.332216Z
270
ihsiang
has-props




















43748

image30.pdf
file




2010-06-01T09:54:22.000000Z
cd629883808115541b95f76ed06d05a1
2010-06-01T10:43:57.332216Z
270
ihsiang
has-props




















52002

image7.pdf
file




2010-06-01T09:54:22.000000Z
1b879dda28e49229dca748b3b14a8c30
2010-06-01T10:43:57.332216Z
270
ihsiang
has-props




















20402

image9.pdf
file




2010-06-01T09:54:22.000000Z
6f270cd978b1e8a7b4a4205d163c2da6
2010-06-01T10:43:57.332216Z
270
ihsiang
has-props




















28204


